Solidago: A Modular Collaborative Scoring Pipeline

This paper presents Solidago, an end-to-end modular pipeline to allow any community of users to collaboratively score any number of entities. Solidago proposes a six-module decomposition. First, it uses pretrust and peer-to-peer vouches to assign trust scores to users. Second, based on participation, trust scores are turned into voting rights per user per entity. Third, for each user, a preference model is learned from the user's evaluation data. Fourth, users' models are put on a similar scale. Fifth, these models are securely aggregated. Sixth, models are post-processed to yield human-readable global scores. We also propose default implementations of the six modules, including a novel trust propagation algorithm, and adaptations of state-of-the-art scaling and aggregation solutions. Our pipeline has been successfully deployed on the open-source platform tournesol.app. We thereby lay an appealing foundation for the collaborative, effective, scalable, fair, interpretable and secure scoring of any set of entities.

==> app-prior.tex <==
\section{The prior weight}
\label{app:prior}
To estimate our prior weight, we need to first learn the individual raw scores with an initial prior weight.
In this paper, we selected a very small initial prior weight, equal to $10^{-8}$.
We then obtain different noise squares, variances and prior weights for the different criteria.
The values are presented in Table~\ref{table:prior_weight}.
Despite some (expectable) fluctuations of the estimate of $\contributorpriorweight$ for the different criteria,
we eventually selected a single value for all criteria, equal to $\contributorpriorweight \triangleq 1$.
This is the value now used in our implementation.
\len{To be updated.}
\begin{table}[h!]
    \centering
    \begin{tabular}{|l|c|c|c|}
    \hline
    Quality criterion $\quality$ & $\hat \sigma_{0 \quality}^2$  & $\hat V_\quality$ & $\contributorpriorweight$ \\ \hline \hline
largely\_recommended   &  $0.181$  &   $0.285$ & $0.634$ \\ \hline
reliability            &  $0.182$  &   $0.148$ & $1.230$ \\ \hline
pedagogy               &  $0.181$  &   $0.164$ & $1.098$ \\ \hline
importance             &  $0.181$  &   $0.273$ & $0.663$ \\ \hline
layman\_friendly       &  $0.184$  &   $0.133$ & $1.384$ \\ \hline
entertaining\_relaxing &  $0.192$  &   $0.189$ & $1.015$ \\ \hline
engaging               &  $0.182$  &   $0.217$ & $0.836$ \\ \hline
diversity\_inclusion   &  $0.189$  &   $0.130$ & $1.459$ \\ \hline
better\_habits         &  $0.186$  &   $0.206$ & $0.907$ \\ \hline
backfire\_risk         &  $0.186$  &   $0.153$ & $1.219$ \\ \hline
    \end{tabular}
    \caption{Prior weight estimates along the different criteria}
    \label{table:prior_weight}
\end{table}
The need of relatively large prior weights was also observed empirically by Tournesol's contributors.
Before adopting such large weights, Tournesol used $\contributorpriorweight = 0.01$. 
This was insufficient, as individual raw scores for alternatives with few comparisons took very diverse values.
In particular, this noise implied that top alternatives for a contributor were often those with few comparisons,
even when the alternatives were not regarded as top alternatives by the contributor.
The modification seems to have increased the contributors' experience, and their trust in Tournesol's algorithm.
In our empirical estimations, we also observed a negative correlation between the number of comparisons provided by a contributor $\contributor$ and the estimate of their noise $\hat \sigma_{\contributor 0}^2$ (see Figure~\ref{fig:correlation_nComparaisons_sigma}).
It is not yet clear how to best explain this phenomenon.
This might be an artefact of our estimator.
Another possible explanation is that contributors improve the consistency of their judgments as they spend more time (and perhaps attention) comparing alternatives.
Future work should aim to clarify this.
\begin{figure}[h!]
    \centering
    \includegraphics[width=.7\linewidth]{correlation_nComparaisons_sigma.png}
    \caption{Correlation between the number of comparisons provided by a contributor and the estimate $\hat \sigma_{n0}^2$}
    \label{fig:correlation_nComparaisons_sigma}
\end{figure}
We also acknowledge that further research is needed to estimate a more appropriate prior weight.
First, our experiments showed that if we repeat the estimate of $\contributorpriorweight$ with an initial value of $1$,
then the new estimate takes ever larger values,
mostly because the variance of the scores then goes to 0.
This is not surprising, as large prior weights indeed force scarcely scored alternatives to have scores close to 0.
We considered that this phenomenon should be discarded when estimating $\contributorpriorweight$, 
hence the use of a very small initial value.
Second, we took the more robust but less accurate decision to only estimate a single $\contributorpriorweight$ for all contributors on all criteria.
Yet, this prior should in fact depend on contributors and criteria, 
as some contributors should be expected to score with significantly less noise than others,
especially on some "easy-to-judge" quality criteria.
However, doing personalized estimates robustly is a nontrivial task, as exposed by the James-Stein paradox~\cite{stein1956variate,james1992estimation}.
